The Magnificent Seven Challenges and Opportunities in Domain-Specific Accelerator Design for Autonomous Systems

The end of Moore's Law and Dennard Scaling has combined with advances in agile hardware design to foster a golden age of domain-specific acceleration. However, this new frontier of computing opportunities is not without pitfalls. As computer architects approach unfamiliar domains, we have seen common themes emerge in the challenges that can hinder progress in the development of useful acceleration. In this work, we present the Magnificent Seven Challenges in domain-specific accelerator design that can guide adventurous architects to contribute meaningfully to novel application domains. Although these challenges appear across domains ranging from ML to genomics, we examine them through the lens of autonomous systems as a motivating example in this work. To that end, we identify opportunities for the path forward in a successful domain-specific accelerator design from these challenges.

==> tex/scratchwork_and_notes.tex <==
\section{Brian's Notes on the Failures We Came Up With}
\begin{itemize}
    \item Isolation from Domain Experts: Understanding what the Customer Wants (gave them the wrong kernel) -- Usability and Communication are key -- need wrappers -- need to meet people where they are
    \item Metrics Matter: Power vs. Latency vs. Throughput With MLPerf the ML people all cared about accuracy -- the systems people increased throughput but at the expense of accuracy -- so then no one cared -- because now you needed to train longer actually -- its time to accuracy not time overall -- Joe Lemer -- benchmarks are important
    \item Widgitism: don't do something SOOOOOO specific -- need to find cross-cutting kernels -- benchmarking for the "real" subkernels
    \item Missing the Forrest for the Trees: One Kernel vs. End-to-End Application
    \item Pump the Brakes, Don't Always Accelerate -- Don't Pretend Your Accelerator is Free -- Data center as a computer vs. one deployment -- super comptuer people said the same thing -- at the HPC level you need system behavior -- you can't do micro scale optimization becuase it kills the scheduler at the macro scale
    \item Flexable Accelerators are Still Accelerators -- GPUs, FPGAs are great -- use them -- software can get you really far and let you get better coverage faster -- (maybe Brian's work?) -- Amdals Law is king and its a moving target -- feedback mechanism
\end{itemize}

\textbf{Brian's other notes follow:}
It’s all the same it’s all different: architecture and systems for embodied autonomy
We want to build domain specific architectures for lots of domains

To do so, we need to find the right layer of abstraction for our domain (high level intermediate representations). VLSI is the same thing -- its done through a comiler -- to make design flows. Genomics and ML maybe?

Widgitism is a problem

Interface with domain exerpts -- learn to speak their language -- and make sure what they care about is included in our stack -- what do they think are core workloads -- but the ones they think are problems are the ones that failed the harware library

Then can develop things (locality, sparisty, concurrency, parallellism, and middlewear/ASICs)

Then at the end there is a feedback mechanism that we will need to fundamental benchmarking applied to those workloads and broaden the space of what is the bottleneck (henry ford on people wanted a "faster horse")

So what did we learn about robotics and other embodied autonomy? End to end matters — benchmarking through middleware — optimization through heterogeneity — accelerating across algorithms

\textbf{Sabrina's notes}
metrics matter
    joel emer + vivienne
    benchmarks!!!

wigitism

disconnect from domain experts

forest vs. trees: end to end views

no such thing as a free lunch: don't always accelerate: unusal accelerators: pump the brakes, don't always accelerte: can use CPU or GPU, or TPUs

ahmdal's law is king: and it's a moving target

tech transfer ++

%---------------------------
% Long initial draft of Sec 3: Future Directions & Opportunities
%---------------------------
\section{Future Directions \& Opportunities}

We envision a future where accelerator design is characterized by close collaboration between domain experts and hardware designers, adaptability to evolving algorithmic landscapes, and a holistic view of the entire system. Central to this vision is the recognition that due to the ever evolving algorithms and workloads, the focus should be on identifying and supporting common, cross-cutting primitives that can be flexibly composed to support holistic systems.
%that effective accelerator design cannot occur in isolation. It requires active engagement and knowledge sharing between experts in the target domain and those in computer architecture. Moreover, the rapid pace of innovation in many such as ML and robotics demands accelerator designs that can adapt to evolving algorithms and workloads. Rather than designing accelerators for a single, static algorithm, the focus should be on identifying and supporting common, cross-cutting primitives that can be flexibly composed to support a range of algorithms within a domain. Finally, a holistic view of the entire system is crucial for effective accelerator design. 

\subsection{Enabling Technologies and Methodologies}

To realize the vision of collaborative, adaptive, and holistic domain-specific accelerator design, several key enabling technologies and methodologies need to be developed and adopted. In this section, we discuss three critical areas: agile design tools, machine learning for system design, and end-to-end modeling and simulation.

\subsubsection{Agile Design Tools}
One key opportunity lies in the development of agile design tools that streamline the creation and customization of domain-specific accelerators (DSAs). These tools should operate at a high level of abstraction, allowing users to specify accelerator functionality through intuitive methods such as domain-specific languages (DSLs) or graphical interfaces, and enabling domain experts to directly participate in the design process. %By lowering the barrier to entry, agile design tools can enable domain experts to directly participate in the accelerator design process, ensuring that the resulting designs accurately capture the unique requirements and constraints of the target domain.

Moreover, agile design tools should strive to bridge the gap between high-level algorithmic specifications and low-level hardware implementations. This can be achieved through the use of formal verification techniques that guarantee the correctness of the generated hardware with respect to the high-level specification. %Additionally, these tools should employ advanced optimization techniques, such as those based on machine learning, to automatically explore the design space and generate efficient hardware implementations. % that approach the performance of hand-crafted designs.

To keep pace with the rapid evolution of algorithms and computing platforms, agile design tools should be modular and extensible. They should allow for the easy integration of new hardware primitives, such as those based on emerging technologies like non-volatile memory or photonics. %This modularity enables designers to quickly explore alternative implementation options and adapt their designs to changing requirements.

\subsubsection{Machine Learning for System Design}

Machine learning (ML) techniques, particularly those based on deep learning and reinforcement learning, have the potential to revolutionize the way we design and optimize domain-specific accelerators. By leveraging the ability of ML models to learn complex patterns and make data-driven decisions, we can automate many of the tedious and time-consuming aspects of the accelerator design process.

One promising application of ML in accelerator design is in the area of design space exploration (DSE). Given a high-level specification of the target algorithm and a set of hardware constraints, an ML model can be trained to search the vast space of possible hardware configurations and identify the most promising candidates, saving time and possibly uncovering unconventional designs that might be overlooked by human designers. %This approach can significantly reduce the time and effort required for DSE, while also potentially discovering novel and unconventional designs that might be overlooked by human designers.

Another area where ML can have a significant impact is in the optimization of accelerator hardware for specific workloads. By analyzing the characteristics of the target application, such as its data access patterns and computational requirements, ML models can suggest optimizations that improve performance, energy efficiency, or other metrics of interest. %This workload-driven optimization approach can lead to accelerators that are highly tuned for specific domains, rather than being generic and suboptimal.

\subsubsection{End-to-End Modeling and Simulation}
To design effective DSAs, it is essential to consider the entire system in which they will be deployed, rather than focusing solely on the accelerator in isolation. This requires end-to-end modeling and simulation tools that can capture the complex interactions between the accelerator, the rest of the computing system, and the physical environment.

A key aspect of end-to-end modeling is the ability to accurately simulate the data flow through the system, from sensors and input devices to the accelerator and back to actuators or output devices. This simulation should take into account the bandwidth and latency constraints, processing delays, and power and thermal characteristics of the system.
%of the various interconnects and memory hierarchies, as well as the processing delays introduced by the accelerator and other system components. In addition to data flow, end-to-end modeling should also consider the power and thermal characteristics of the system. This includes the power consumption of the accelerator itself, as well as the impact of the accelerator on the power and thermal budgets of the overall system. 
%By accurately modeling these factors, designers can make informed decisions about the placement and integration of the accelerator within the system, as well as the necessary power and thermal management strategies.
%
Finally, end-to-end modeling should consider the physical environment in which the system will be deployed. For example, in the case of an autonomous vehicle, the model should take into account factors such as the vehicle dynamics, sensor noise, and weather conditions. Combined, this information will enable designers to develop robust and reliable real world accelerators.
% By incorporating these environmental factors into the simulation, designers can gain a more realistic understanding of how the accelerator will perform in the real world, and can make necessary adjustments to ensure robust and reliable operation.



% One key opportunity lies in the development of agile design tools that streamline the creation and customization of DSAs.
% %
% The ideal agile design tool would operate at a high level of abstraction, allowing users to specify accelerator functionality through intuitive methods such as domain-specific programming languages (DSLs) or even graphical interfaces, lowering the barrier to entry for new participants.
% %
% Furthermore, these tools should strive to bridge the gap between designer intent and hardware reality. Ideally, they would leverage formal verification techniques to ensure the generated hardware design accurately reflects the high-level specifications, guaranteeing correctness and reducing the risk of errors. Additionally, these tools should aim to produce designs that approach the performance of meticulously hand-crafted accelerators by employing advanced optimization algorithms and leveraging knowledge of the target domain and hardware capabilities.
% %
% To address the ever-evolving landscape of hardware innovation, agile design tools should exhibit a high degree of modularity. This would allow for the seamless integration of modules that represent emerging hardware paradigms like in-memory processing units, neuromorphic computing engines, or even quantum computing architectures. 
% %
% By incorporating these modules, designers could explore a wider design space and create optimal systems that leverage the most suitable hardware building blocks for a given task and quickly and effectively iterate to keep pace with the ever evolving algorithmic landscape in many domains.
% %
% \todo{(Add some concrete examples of projects that have kind of done this.)}

% \noindent\textbf{Machine Learning for System Design.} These tools can be further empowered by harnessing the potential of machine learning (ML) techniques, particularly generative AI, which can theoretically enable real-time exploration of a vast design space hardware designs, as well as the creation of novel hardware architectures.
% %
% The impact of ML extends beyond accelerator design itself. Machine learning algorithms can be employed to automate various aspects of the design process.
% For example, ML models could analyze high-level specifications written in DSLs and suggest optimizations or identify potential bottlenecks early in the design flow. Machine learning can also potentially be utilized to develop more efficient and comprehensive verification techniques, ensuring the functional correctness of the generated hardware designs. Finally, through ML, design tools could adapt to user preferences over time, personalizing the design experience.
% %
% \todo{(Add some concrete examples of projects that have kind of done this.)}

%\noindent\textbf{End-to-End Modeling and Simulation.}
%A holistic approach to accelerator design demands the consideration of pre- and post-processing stages within the system. Measuring and optimizing the entire processing pipeline, not just the isolated accelerator itself, will ensure that performance gains are not negated by inefficiencies elsewhere in the system. This necessitates full-system integration efforts by interdisciplinary teams that can account for data flow, memory access patterns, and overall system power consumption.

\subsection{Fostering a Robust Research Ecosystem}

Realizing the vision of collaborative, adaptive, and holistic domain-specific accelerator design requires more than just technical advances. It also depends on fostering an ecosystem that encourages collaboration, knowledge sharing, and innovation. 

\subsubsection{Cross-Domain Collaboration}
Accelerator design is inherently a multidisciplinary endeavor, requiring expertise from a wide range of fields, including computer architecture, electronic design automation, compiler optimization, machine learning, and domain-specific knowledge. To facilitate collaboration between these diverse communities, it is essential to establish dedicated forums for knowledge sharing and exchange. An effective way to promote cross-domain collaboration is through the organization of specialized workshops and conferences that bring together researchers and practitioners from different fields. These events provide an opportunity for participants to share their latest findings, discuss common challenges and opportunities, and explore potential collaborations. For example, a workshop on ``Machine Learning for Accelerator Design'' could bring together experts in computer architecture, ML, and EDA to explore how ML techniques can be applied to the design and optimization of domain-specific accelerators.

In addition to workshops and conferences, cross-domain collaboration can be facilitated through the creation of interdisciplinary research centers and consortia. These organizations can provide a platform for researchers from different institutions and domains to work together on common projects, share resources and infrastructure, and jointly develop new technologies and methodologies.

\subsubsection{Open-Source Resources}
A key element of a robust research ecosystem is the availability of open-source resources, including software tools, hardware designs, and datasets. By making these resources freely available to the research community, we can lower the barriers to entry for new researchers, enable reproducibility and comparability of results, and accelerate the pace of innovation.

Open-source datasets and benchmarks are  critical for advancing the field of accelerator design. By providing curated and well-characterized datasets that are representative of real-world workloads, we can enable researchers to evaluate their designs under realistic conditions and compare their results against those of other researchers. An example of such a dataset is the ILLIXR benchmark suite, which provides a set of AR/VR workloads for evaluating the performance and power efficiency of accelerator designs.

Another area where open-source resources can have a significant impact is in the development of agile design tools for accelerator design. By creating open-source frameworks and libraries for high-level synthesis, design space exploration, and hardware-software co-design, we can enable researchers to quickly prototype and evaluate new accelerator designs without having to start from scratch. Another important type of open-source resource is reference designs and implementations of domain-specific accelerators. By making these designs available to the community, along with detailed documentation and performance data, we can enable researchers to build upon and compare against state-of-the-art designs. This can help to establish a common baseline for evaluation and promote the sharing of best practices and design techniques.

\subsubsection{Standardized Benchmarks and Metrics}
To enable meaningful comparison and evaluation of accelerator designs, it is essential to establish standardized benchmarks and metrics that are widely accepted by the research community. These benchmarks should be representative of the workloads and use cases that are most relevant to the target domain, and should cover a range of performance, power, and area targets. One example of a standardized benchmark suite for machine learning accelerators is MLPerf, which provides a set of reference workloads and evaluation criteria for measuring the performance of ML training and inference systems. By using a common set of benchmarks and metrics, researchers can compare their designs against those of others in the field and track progress over time. In addition to performance benchmarks, it is also important to establish standardized metrics for evaluating the energy efficiency, cost, and other key characteristics of accelerator designs. 

Representative, fair and effective benchmarks can help to ensure that accelerators are not only fast, but also efficient and cost-effective, which is critical for their adoption in real-world systems. Finally, standardized benchmarks and metrics can also play a key role in driving innovation and guiding research priorities. By identifying the most important and challenging workloads and use cases, benchmarks can help to focus research efforts on the areas that are most likely to have a significant impact. Similarly, by establishing clear and measurable targets for performance, efficiency, and other key metrics, benchmarks can provide a roadmap for progress and help to accelerate the pace of innovation in the field.



%\noindent\textbf{Community Infrastructure and Democratizing Design.}
%A critical opportunity lies in fostering a robust and collaborative research ecosystem. This can be achieved through the establishment of dedicated cross-domain workshops, joint interdisciplinary conferences, and the creation of a rich pool of open-source resources. Shared resources could encompass standardized benchmarks, open-source infrastructure and codebases (e.g., widely popular projects in robotics and architecture such as ROS~\cite{quigley2009ros} and MLIR~\cite{lattner2021mlir}). Importantly these resources need to provide comprehensive documentation and avoid language-specific dependencies to enable flexibile analysis and usage. Such collaborations would accelerate progress by enabling researchers to build community, collaborative ideas and projects, and avoid duplicating efforts.

%The development of effective and standardized benchmarks is paramount. These benchmarks should go beyond raw performance metrics and encompass factors such as power consumption, memory usage, and real-time response characteristics. By establishing a common ground for evaluating and comparing accelerators, researchers can ensure that designs are optimized for the specific needs of autonomous systems.
%
%\todo{(Add some concrete examples of projects that have kind of done this.)}


\subsection{Sustainable and Responsible Acc. Design}

It is increasingly important to consider the environmental and societal impacts of accelerator design. Sustainable and responsible accelerator design encompasses a broader range of considerations, including materials and fabrication processes, strategic deployment, lifecycle analysis, and end-of-life management.

\subsubsection{Materials and Fabrication Processes}
In addition to energy consumption, the materials and fabrication processes used in accelerator design can also have significant environmental impacts. For example, the production of silicon wafers and the use of toxic chemicals in semiconductor manufacturing can contribute to air and water pollution, as well as greenhouse gas emissions. To mitigate these impacts, it is important to explore alternative materials and fabrication processes that are more sustainable and environmentally friendly. In addition, the development of new fabrication processes, such as additive manufacturing and 3D monolithic architectures, can enable the production of accelerators with less waste and fewer toxic chemicals. These processes can also enable the creation of more complex and customized accelerator designs, which can help improve performance and energy efficiency.

\subsubsection{Strategic Deployment of Accelerators}
While accelerators can provide significant benefits in performance and energy efficiency for specific workloads, it is important to carefully consider the scenarios in which they are deployed. In some cases, the use of accelerators may not provide sufficient benefits to justify their cost and complexity, particularly for workloads that are not well-suited to acceleration. Therefore, it is important to conduct thorough analysis and modeling to determine the specific scenarios in which accelerators can provide significant advantages over general-purpose computing solutions. This analysis should take into account not only the performance and energy efficiency of the accelerator, but also factors such as the cost of development and deployment, the scalability and flexibility of the solution, and the potential for reuse across multiple applications and domains. By strategically deploying accelerators in the scenarios where they can provide the greatest benefits, we can help to ensure that the costs and environmental impacts of accelerator development are justified by the resulting improvements in performance and efficiency. This can also help to avoid the proliferation of specialized hardware that may have limited applicability and a short lifespan, which can contribute to electronic waste and other environmental concerns.

\subsubsection{Lifecycle Analysis and End-of-Life Management} Sustainable and responsible accelerator design requires considering the entire lifecycle of the hardware, from raw materials extraction to end-of-life management. This includes the design phase, manufacturing, use, and eventual disposal or recycling of the accelerator. Lifecycle analysis (LCA) is a powerful tool for assessing the environmental impacts of a product or system throughout its entire lifespan. By conducting LCA for accelerator designs, researchers and engineers can identify opportunities for reducing the environmental footprint of the hardware, such as selecting low-impact materials, optimizing manufacturing processes, or designing for easier disassembly and recycling. Effective end-of-life management is also crucial for minimizing the environmental impact of accelerators. This includes the development of efficient recycling processes for recovering valuable materials, such as precious metals and rare earth elements, from discarded hardware. It also involves the safe disposal of toxic or hazardous materials, such as lead and mercury, which can pose significant health and environmental risks if not handled properly.

By adopting a lifecycle perspective and prioritizing sustainability throughout the design, manufacture, use, and disposal of accelerators, we can help ensure that the benefits of these technologies are realized without compromising our planet and future generations.



%-----------------------------------------------------------
%\textbf{Building a Collaborative Ecosystem:} 
%\textbf{Metrics that Matter:} 
%\textbf{Expanding the Design Toolbox:}
%The exploration of a broader range of heterogeneous design options will be needed to develop flexible and general solutions. Cost models, similar to those employed in datacenter design (e.g.,~\cite{greenberg2008cost}), can be leveraged to assess the viability of alternative approaches like FPGAs and domain-specific architectures. Careful consideration should also be given to Non-Recurring Engineering (NRE) costs associated with various design choices, ensuring a holistic evaluation that acknowledges the ``no free lunch'' principle. As the field matures, the concept of a linear progression from CPUs to GPUs to FPGAs and finally to ASICs may need to be revisited. Research into alternative accelerator architectures, particularly those that offer a balance between flexibility and performance, holds promise for specific applications within the autonomous systems domain.
%%\textbf{End-to-End Optimization:} 
%\textbf{Sustainability by Design:} 
%-----------------------------------------------------------

% 2.1 - community/workshops/joint-conferences
% Shared open-source resources
% - benchmarks
% - shared infra/code soures (ROS, OMPL, etc.)
% - no python

% - documentation 
% - 

% 2.2 (metrics matter)
% - benchmarks

% 2.3 (widetism)
% - accelerator cost models (a la datacenters-- Hamilton)
% - think about nre aspects for widgets
% - no free lunch point

% 2.4  (pump the brakes)
% - 

% 2.5 (more than just asics)
% - cpu -> gpu -> fpga -> acceleartors?

% 2.6 (end-to-end)
% - measure pre- and post-processing
% - full-system integration

% 2.7 (sustainability)
% - datacenter on wheels
% - Put the chasing carbon modeling work here somewhere

% These challenges present a series of future opportunities for new research directions, methods, and designs. A bunch of solutions go here.

% \todo{(Something about building ongoing communities through consortiums, open-source living benchmarks and leaderboards (MLPerf and RobotPerf), and workshops and competitions?)}
